A Stochastic Covariance Shrinkage Approach in Ensemble Transform Kalman Filtering

The Ensemble Kalman Filters (EnKF) employ a Monte-Carlo approach to represent covariance information, and are affected by sampling errors in operational settings where the number of model realizations is much smaller than the model state dimension. To alleviate the effects of these errors EnKF relies on model-specific heuristics such as covariance localization, which takes advantage of the spatial locality of correlations among the model variables. This work proposes an approach to alleviate sampling errors that utilizes a locally averaged-in-time dynamics of the model, described in terms of a climatological covariance of the dynamical system. We use this covariance as the target matrix in covariance shrinkage methods, and develop a stochastic covariance shrinkage approach where synthetic ensemble members are drawn to enrich both the ensemble subspace and the ensemble transformation. We additionally provide for a way in which this methodology can be localized similar to the state-of-the-art LETKF method, and that for a certain model setup, our methodology significantly outperforms it.

==> Prereview/header.tex <==
\newcommand\1{\one}
\def\!#1{\mathcal{#1}}
\def\*#1{\boldsymbol{\mathbf{#1}}}
\def\|#1{\textnormal{#1}}
\def\##1{\mathpzc{#1}}
\renewcommand{\Re}{\mathds{R}}

\def\det#1{\left\lvert#1\right\rvert}
\def\norm#1{\left\lVert#1\right\rVert}
\def\diff#1{\mathrm{d}#1}
\def\sgn{\text{sgn}}

\def\pss#1#2{\prescript{}{#1}{#2}}
\def\psss#1#2#3{\prescript{#1}{#2}{#3}}

\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\tr}{tr}

\newcommand{\C}[2]{\*\Sigma_{#1#2}}
\newcommand{\Ct}[2]{\widetilde{\*\Sigma}_{#1#2}}
\newcommand{\Bt}{\widetilde{\*B}}

\newcommand{\xf}{X^\|f}
\newcommand{\cxf}{\!X^\|f}
\newcommand{\bxf}{\*X^\|f}


%\DeclareMathOperator{\tr}{tr}

\newcommand{\Id}{\mathbf{I}}
\newcommand{\R}{\mathbf{R}}
\renewcommand{\S}{\mathbf{S}}
\newcommand{\transp}{\mathsf{T}}
\newcommand{\Tp}{\mathsf{T}}

\newtheorem{remark}{Remark}

\usepackage{caption}
\usepackage{subcaption}

==> Prereview2/header.tex <==
\newcommand\1{\one}
\def\!#1{\mathcal{#1}}
\def\*#1{\boldsymbol{\mathbf{#1}}}
\def\|#1{\textnormal{#1}}
\def\##1{\mathpzc{#1}}
\renewcommand{\Re}{\mathds{R}}

\def\det#1{\left\lvert#1\right\rvert}
\def\norm#1{\big\lVert#1\big\rVert}
\def\diff#1{\mathrm{d}#1}
\def\sgn{\text{sgn}}

\def\pss#1#2{\prescript{}{#1}{#2}}
\def\psss#1#2#3{\prescript{#1}{#2}{#3}}

\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\tr}{tr}

\newcommand{\C}[2]{\*\Sigma_{#1#2}}
\newcommand{\Ct}[2]{\widetilde{\*\Sigma}_{#1#2}}
\newcommand{\Bt}{\widetilde{\*B}}

\newcommand{\xf}{X^\|f}
\newcommand{\cxf}{\!X^\|f}
\newcommand{\bxf}{\*X^\|f}


%\DeclareMathOperator{\tr}{tr}

\newcommand{\Id}{\mathbf{I}}
\newcommand{\R}{\mathbf{R}}
\renewcommand{\S}{\mathbf{S}}
\newcommand{\transp}{\mathsf{T}}
\newcommand{\Tp}{\mathsf{T}}

\newtheorem{remark}{Remark}

\usepackage{caption}
\usepackage{subcaption}

==> Prereview2/responsetorev.tex <==
Response to reviewer 1

"Concepts like KL Kullback-Leibler divergence are not necessarily familiar to atmospheric scientists and this applies to other concepts in the ms. The same applies for the Rao-Blackwellized Ledoit-Wolf (RBLW) estimator."

Answer: The explanation of the RBLW estimator has been substantially expanded in section 2. A line has been added to indicate that the low KL divergence would indicate an ensemble representative of the truth.

"The opinion of this reviewer is that the present manuscript is much more suitable to a scientific computational journal such as SIAM journal of Scientific Computing as it lacks meteorological specificity. ... As an alternative they should consider testing their method on a  meteorological realistic WRF-LETKF system for experiments with real observations which can be considered a major revision required for acceptance for publication in Tellus."

Tellus A has on multiple occasions published new ensemble Kalman filter methods that were tested on Lorenz '96 and the QGE (For example see "Pavel Sakov and Peter R Oke. A deterministic formulation of the ensemble Kalman filter: an alternative to ensemble square root filters. 2008."). It is our opinion that the manuscript and the methodology is well suited for publication to Tellus A.

Response to reviewer 2:

"1) Throughout, the paper is vague and omits important details. The shrinkage approach
relies heavily on the choice of target matrix P, but the authors do not explain how the
target is/should be chosen and what the effects of a poor choice are. I believe that with
a “poor” choice of target, even a “good” gamma cannot yield good results. For that
reason, localizing the target, which in numerical experiments seems to be based on
climatological estimates, should be carefully tuned, but this is not explained."

Sections 2 and 3 have been significantly expanded to clarify both the background, and the proposed approach. A discussion about the choice of target matrix was added to the end of section 2.

"2) In numerical experiments, the authors discuss several variants of the proposed
shrinkage approach, but the paper would be stronger if the authors also compare to
“classical” localization methods — is the shrinkage approach useful compared to a
“vanilla” LETKF, classically tuned (i.e., varying the localization radius and optimizing
forecast error)? Moreover, the numerical tests are done with relatively simple models
(L95 and QG) and a discussion is necessary as to what conclusions one can draw from
these simplified numerical experiments."

The QG experiments already compare our method against an optimally tuned LETKF with Gaspari-Cohn localization. We have added a line to indicate that the GC radius has been optimally tuned.


"3) Section 2.3: I was looking forward to learning about shrinkage techniques, but I found
myself puzzled at the end of this section. I understand the authors have a lot of
experience with shrinkage methods, but the paper would be more impactful and easier
to read (independently of other papers) if the basic ideas of shrinkage methods would
be explained in more detail. Please consider adding more explanations to this important
background section. Specifically, I am unsure how to “choose” a target matrix P and
what the consequences of specific choices could be (see above)."

As is the reply to point 1, the sections on covariance shrinkage and our methodology have been significantly expanded, and rewritten. It is the authors' hope that readers coming from a meteorology background will now gain a better understanding of the proposed methodology.


"1) Consider using a different greek letter in (2.1), I find this letter hard to read and to use
when taking notes (but this is stylistic and can be neglected)."

We did change the capital "Xi" to the small letter "xi", in hope of improving readability. The authors believe that the letter "Xi" is commonly used for the notation involving model error. (equation 2.1)

"2) P. 4 Lines 21-40: Please explain this approximation in more detail and/or give
references."

The authors have found no reference to this in the literature. The discussion of this approximation has been replaced by a simple statement, as to not distract from the rest of the paper.

"3) P. 4 Line 52: What do you mean by “perfect”? Please be more scientifically accurate
and less colloquial."

We have reworded to "inexact". (See line 66)

"3) P. 5 Line 19: The term “shrinkage” is used here (and again, colloquially referred to
as “a type of”), but it is not yet clear/explained what this is. Please remove or explain."

We have removed this line.

"4) P.5 Lines 60-61: There seems to be some confusion between covariances and
correlations. Please correct."

All terms related to covariance matrices have been changed to "covariances". All terms related to localization have keep the terms "correlation" (1 appearance in the abstract) or "decorrelation" (14 appearances in the text), as this is the correct common terminology when refering to such.

"5) Equation 2.14: Please give more background about how this gamma is chosen, in
particular in what sense this choice is “optimal” (what is optimized here?)."

We have added a line to indicate what this is estimating (see line 107) 

"6) Equation 2.16: It is stated that the choice of gamma is “extremely important”. Please
explain in what way the reader should interpret “extremely important” and what the
advantages are of using (2.16) over (2.14) etc."

We have expanded the discussion regarding the significance of gamma, and regarding the advantages and downsides of the RBLW estimator (see lines 121-141)

"7) P. 7 Lines 6-17: You describe two major issues. How do the proposed algorithms
deal with these issues?"

The text (lines 134 to 141) should now hopefully make it clear that we are describing drawbacks to using our proposed methodology without providing a clear answer as to show these issues can be avoided.

"8) P.7 Lines 18-26: In my experience, the “cut-off”, r, has a drastic influence on the
results. How should r be chosen? How is this done in the numerical experiments?
Please consider adding detailed explanations here."

We have added a line to indicate that the localization radius for GC has been optimally tuned. (see lines 311)

"9) P.7 Lines 38-45: What is “our” uncertainty and why is climatological information
“locally known”? I have trouble interpreting these sentences, please clarify."

"Our uncertainty" refers to the Bayesian interpretation of inference. It is inherently dependent on the knowledge of the agent (be it human or machine) performing the inference, thus "our knowledge" and "our uncertainty". This is the terminology used in some statistical literature. The text "locally known" has been removed and largely replaced by "historical". (see line 158 for example)

"10) P.8 Line 17: There is a contradiction. You assume that you know the covariance,
but you want to get to this covariance using localization. Please clarify this circular
reasoning."

We are not sure as to what this is referring to. We see no contradiction. The target covariance, and thereby all forecast ensembles are known prior to the calculation of the shrinkage covariance estimate.

"11) P.8 Lines 25-16: Consider removing the part about Laplace assumptions. It may be
“obvious” to the authors, but this paragraph is not useful for many of Tellus’ readers."

We agree, this has been removed. 

"12) Equation 3.5: How do you pick gammai? Are there general guidelines, a general
tuning framework etc? Please add some clarification here."

We have added the line that in this paper this is the RBLW estimate of gamma. (line 196)

"13) Your use of remarks (p.11 and 16): Consider not using the “Remark” framework,
which is mathematical and it seems out of place of the rest of this paper."

The remark notation has been removed, and the remarks now appear in-text.

"14) L96 assimilation results: I am not sure what is compared here and what “optimal” is
referring to (lines 31 and 34, p. 13). The paper would be stronger if the authors not only
compare variants of the shrinkage techniques, but also compare to “usual localization,”
e.g., and ETKF or similar algorithm."

The usual localization comparisons are already done with the QGE, see figure 3. We have not shied away from showing that the LETKF under certain configurations does in fact beat our method purely in terms of error (see 308-315)

"15) P.14 Line 26: how are the dynamic ensemble sizes modified? Please explain."

We are not sure what this is referring to. If it is referring to the methodology, then the dynamical ensemble size (N) is fixed for all time. We have not considered the case of a changing dynamical ensemble size. If this is refering to the experiments section (section 4), then the ensemble sized are iterated over, and RMSE (and KL) results are obtained for distinct combinations of N and other factors considered.

"16) P. 14, line 30: why/how are gamma values “produced”? Please explain."

The factor gammai, unless otherwise specified to be constant, is computed with the RBLW estimator (see line 196)

"17) The QG model: I believe this is a model on a 2D domain?"

This is stated in the paper. (line 285)

"18) P.15 Line 11: When you apply Gaspari-Cohn to localize (and thereby define the
target matrix P?), how is the spatial length scale of the Gaspari-Cohn function tuned?"

We have added a line to describe that the localization radius is optimally tuned. (line 311)

"19) P.15 Line 13: “Nature” - do you mean the journal, our environment, or a run with the
model that is used to generate observations? Please specify your terminology more
clearly."

We believe that "Nature" is standard terminology in data assimilation literature, and is used to refer to the "true" physical reality, and more specifically to the "true" physical system under consideration.

"20) P.15, Lines 39-43: This statement about ETKF is wrong (and violated by the L96
setup described in this paper). It is in fact the opposite. During a local analysis, nearby
grid points use a very similar set of observations so that the analysis remains (more or
less) smooth."

While the reviewer's statement might be true for some operational models with very sparse observations, for QGE with dense observations, this is not the authors' experience. A naive local update will simply fail as there will be large discontinuities in the solution, leading to non-physical velocities in the QGE. This might be in large part due to the large observation errors in our experiments, and the relative closeness of the observations, but nonetheless our experimental setup is standard for looking at the QGE (see Sakov and Oke 2008). The reason for the inclusion of an "operational approximation" localization function is to attempt to mimic the behavior the reviewer describes in our formulation, and not have a method that simply does not work (as the alternative would in fact lead to an empty plot). Lines 297-306 have been clarified to explain this phenomenon.


"21) P. 15 Line 46: What do you mean by “unfair”? Please focus on strategies that are
reasonable and that are in scientific use. Applying these is not “unfair”."

We have reworded the sentence to reflect the answer above. (lines 297-306)

"22) Equation 4.7: What happens for k>5/4? What is “const”?"

This is a typo, it should have read "sonst." We have changed it to "otherwise" to be consistent with newer English conventions. (equation 4.7)

"23) P. 16, line 7: “handily beats” — how do I see this from the figure and what does this
mean? Please be more specific in your explanations."

The word handily has been removed and the sentence clarified. (lines 308-326)

"24) P.16 Lines 7-20: Is there a reason for why the shrinkage approach should be
expected to do better for nonlinear observations? The rest of this paper does not make
this point and I am not sure this is justified by the theoretical and numerical
developments."

We have changed the wording to reflect a much weaker state of affair, merely that the methodology can work for non-linear observations. (see lines 319-322)


"25) P. 16 Lines 22-32: Again, how is gamma chosen? I understand the choice is
“extremely important”, but it is not clear how the authors propose to choose gamma."

We believe that this is adequately explained in the paper. (see line 196)

"26) Acknowledgements: I am not aware that this paper has already been reviewed by P.
Sakov and another reviewer, I see it for the first time."

This draft is a resubmission, thus it has already been reviewed and substantially changed once.

"27) The appendix is not mentioned in the text and, for that reason, perhaps not needed.
(I did not read/review the appendix since it was never mentioned)."

The appendix has been removed.

"28) Throughout the numerical experiments: when you refer to RMSE, do you mean
analysis RMSE or forecast RMSE?"

We have corrected the formula and clarified that this is in fact the analysis RMSE. (equation 4.3)

"29) Since this paper is about using shrinkage to localize ensemble filters, I recommend
to revise the title to reflect that localization is a key issue here."

While shrinkage does attempt to apply similar ideas to those under the umbrella term "localization", we believe that the methodology is sufficiently different as to merit being described by its own name; we believe that the title is accurate for the methodology, and thus will keep the name.

==> Reviews_Tellus_v1/responsetorev.tex <==
Response to reviewer 1

"Concepts like KL Kullback-Leibler divergence are not necessarily familiar to atmospheric scientists and this applies to other concepts in the ms. The same applies for the Rao-Blackwellized Ledoit-Wolf (RBLW) estimator."

Answer: The explanation of the RBLW estimator has been substantially expanded in section 2. A line has been added to indicate that the low KL divergence would indicate an ensemble representative of the truth.

"The opinion of this reviewer is that the present manuscript is much more suitable to a scientific computational journal such as SIAM journal of Scientific Computing as it lacks meteorological specificity. ... As an alternative they should consider testing their method on a  meteorological realistic WRF-LETKF system for experiments with real observations which can be considered a major revision required for acceptance for publication in Tellus."

Tellus A has on multiple occasions published new ensemble Kalman filter methods that were tested on Lorenz '96 and the QGE (For example see "Pavel Sakov and Peter R Oke. A deterministic formulation of the ensemble Kalman filter: an alternative to ensemble square root filters. 2008."). It is our opinion that the manuscript and the methodology is well suited for publication to Tellus A.

Response to reviewer 2:

"1) Throughout, the paper is vague and omits important details. The shrinkage approach
relies heavily on the choice of target matrix P, but the authors do not explain how the
target is/should be chosen and what the effects of a poor choice are. I believe that with
a “poor” choice of target, even a “good” gamma cannot yield good results. For that
reason, localizing the target, which in numerical experiments seems to be based on
climatological estimates, should be carefully tuned, but this is not explained."

Sections 2 and 3 have been significantly expanded to clarify both the background, and the proposed approach. A discussion about the choice of target matrix was added to the end of section 2.

"2) In numerical experiments, the authors discuss several variants of the proposed
shrinkage approach, but the paper would be stronger if the authors also compare to
“classical” localization methods — is the shrinkage approach useful compared to a
“vanilla” LETKF, classically tuned (i.e., varying the localization radius and optimizing
forecast error)? Moreover, the numerical tests are done with relatively simple models
(L95 and QG) and a discussion is necessary as to what conclusions one can draw from
these simplified numerical experiments."

The QG experiments already compare our method against an optimally tuned LETKF with Gaspari-Cohn localization. We have added a line to indicate that the GC radius has been optimally tuned.


"3) Section 2.3: I was looking forward to learning about shrinkage techniques, but I found
myself puzzled at the end of this section. I understand the authors have a lot of
experience with shrinkage methods, but the paper would be more impactful and easier
to read (independently of other papers) if the basic ideas of shrinkage methods would
be explained in more detail. Please consider adding more explanations to this important
background section. Specifically, I am unsure how to “choose” a target matrix P and
what the consequences of specific choices could be (see above)."

As is the reply to point 1, the sections on covariance shrinkage and our methodology have been significantly expanded, and rewritten. It is the authors' hope that readers coming from a meteorology background will now gain a better understanding of the proposed methodology.


"1) Consider using a different greek letter in (2.1), I find this letter hard to read and to use
when taking notes (but this is stylistic and can be neglected)."

We did change the capital "Xi" to the small letter "xi", in hope of improving readability. The authors believe that the letter "Xi" is commonly used for the notation involving model error. (equation 2.1)

"2) P. 4 Lines 21-40: Please explain this approximation in more detail and/or give
references."

The authors have found no reference to this in the literature. The discussion of this approximation has been replaced by a simple statement, as to not distract from the rest of the paper.

"3) P. 4 Line 52: What do you mean by “perfect”? Please be more scientifically accurate
and less colloquial."

We have reworded to "inexact". (See line 66)

"3) P. 5 Line 19: The term “shrinkage” is used here (and again, colloquially referred to
as “a type of”), but it is not yet clear/explained what this is. Please remove or explain."

We have removed this line.

"4) P.5 Lines 60-61: There seems to be some confusion between covariances and
correlations. Please correct."

All terms related to covariance matrices have been changed to "covariances". All terms related to localization have keep the terms "correlation" (1 appearance in the abstract) or "decorrelation" (14 appearances in the text), as this is the correct common terminology when refering to such.

"5) Equation 2.14: Please give more background about how this gamma is chosen, in
particular in what sense this choice is “optimal” (what is optimized here?)."

We have added a line to indicate what this is estimating (see line 107) 

"6) Equation 2.16: It is stated that the choice of gamma is “extremely important”. Please
explain in what way the reader should interpret “extremely important” and what the
advantages are of using (2.16) over (2.14) etc."

We have expanded the discussion regarding the significance of gamma, and regarding the advantages and downsides of the RBLW estimator (see lines 121-141)

"7) P. 7 Lines 6-17: You describe two major issues. How do the proposed algorithms
deal with these issues?"

The text (lines 134 to 141) should now hopefully make it clear that we are describing drawbacks to using our proposed methodology without providing a clear answer as to show these issues can be avoided.

"8) P.7 Lines 18-26: In my experience, the “cut-off”, r, has a drastic influence on the
results. How should r be chosen? How is this done in the numerical experiments?
Please consider adding detailed explanations here."

We have added a line to indicate that the localization radius for GC has been optimally tuned. (see lines 311)

"9) P.7 Lines 38-45: What is “our” uncertainty and why is climatological information
“locally known”? I have trouble interpreting these sentences, please clarify."

"Our uncertainty" refers to the Bayesian interpretation of inference. It is inherently dependent on the knowledge of the agent (be it human or machine) performing the inference, thus "our knowledge" and "our uncertainty". This is the terminology used in some statistical literature. The text "locally known" has been removed and largely replaced by "historical". (see line 158 for example)

"10) P.8 Line 17: There is a contradiction. You assume that you know the covariance,
but you want to get to this covariance using localization. Please clarify this circular
reasoning."

We are not sure as to what this is referring to. We see no contradiction. The target covariance, and thereby all forecast ensembles are known prior to the calculation of the shrinkage covariance estimate.

"11) P.8 Lines 25-16: Consider removing the part about Laplace assumptions. It may be
“obvious” to the authors, but this paragraph is not useful for many of Tellus’ readers."

We agree, this has been removed. 

"12) Equation 3.5: How do you pick gammai? Are there general guidelines, a general
tuning framework etc? Please add some clarification here."

We have added the line that in this paper this is the RBLW estimate of gamma. (line 196)

"13) Your use of remarks (p.11 and 16): Consider not using the “Remark” framework,
which is mathematical and it seems out of place of the rest of this paper."

The remark notation has been removed, and the remarks now appear in-text.

"14) L96 assimilation results: I am not sure what is compared here and what “optimal” is
referring to (lines 31 and 34, p. 13). The paper would be stronger if the authors not only
compare variants of the shrinkage techniques, but also compare to “usual localization,”
e.g., and ETKF or similar algorithm."

The usual localization comparisons are already done with the QGE, see figure 3. We have not shied away from showing that the LETKF under certain configurations does in fact beat our method purely in terms of error (see 308-315)

"15) P.14 Line 26: how are the dynamic ensemble sizes modified? Please explain."

We are not sure what this is referring to. If it is referring to the methodology, then the dynamical ensemble size (N) is fixed for all time. We have not considered the case of a changing dynamical ensemble size. If this is refering to the experiments section (section 4), then the ensemble sized are iterated over, and RMSE (and KL) results are obtained for distinct combinations of N and other factors considered.

"16) P. 14, line 30: why/how are gamma values “produced”? Please explain."

The factor gammai, unless otherwise specified to be constant, is computed with the RBLW estimator (see line 196)

"17) The QG model: I believe this is a model on a 2D domain?"

This is stated in the paper. (line 285)

"18) P.15 Line 11: When you apply Gaspari-Cohn to localize (and thereby define the
target matrix P?), how is the spatial length scale of the Gaspari-Cohn function tuned?"

We have added a line to describe that the localization radius is optimally tuned. (line 311)

"19) P.15 Line 13: “Nature” - do you mean the journal, our environment, or a run with the
model that is used to generate observations? Please specify your terminology more
clearly."

We believe that "Nature" is standard terminology in data assimilation literature, and is used to refer to the "true" physical reality, and more specifically to the "true" physical system under consideration.

"20) P.15, Lines 39-43: This statement about ETKF is wrong (and violated by the L96
setup described in this paper). It is in fact the opposite. During a local analysis, nearby
grid points use a very similar set of observations so that the analysis remains (more or
less) smooth."

While the reviewer's statement might be true for some operational models with very sparse observations, for QGE with dense observations, this is not the authors' experience. A naive local update will simply fail as there will be large discontinuities in the solution, leading to non-physical velocities in the QGE. This might be in large part due to the large observation errors in our experiments, and the relative closeness of the observations, but nonetheless our experimental setup is standard for looking at the QGE (see Sakov and Oke 2008). The reason for the inclusion of an "operational approximation" localization function is to attempt to mimic the behavior the reviewer describes in our formulation, and not have a method that simply does not work (as the alternative would in fact lead to an empty plot). Lines 297-306 have been clarified to explain this phenomenon.


"21) P. 15 Line 46: What do you mean by “unfair”? Please focus on strategies that are
reasonable and that are in scientific use. Applying these is not “unfair”."

We have reworded the sentence to reflect the answer above. (lines 297-306)

"22) Equation 4.7: What happens for k>5/4? What is “const”?"

This is a typo, it should have read "sonst." We have changed it to "otherwise" to be consistent with newer English conventions. (equation 4.7)

"23) P. 16, line 7: “handily beats” — how do I see this from the figure and what does this
mean? Please be more specific in your explanations."

The word handily has been removed and the sentence clarified. (lines 308-326)

"24) P.16 Lines 7-20: Is there a reason for why the shrinkage approach should be
expected to do better for nonlinear observations? The rest of this paper does not make
this point and I am not sure this is justified by the theoretical and numerical
developments."

We have changed the wording to reflect a much weaker state of affair, merely that the methodology can work for non-linear observations. (see lines 319-322)


"25) P. 16 Lines 22-32: Again, how is gamma chosen? I understand the choice is
“extremely important”, but it is not clear how the authors propose to choose gamma."

We believe that this is adequately explained in the paper. (see line 196)

"26) Acknowledgements: I am not aware that this paper has already been reviewed by P.
Sakov and another reviewer, I see it for the first time."

This draft is a resubmission, thus it has already been reviewed and substantially changed once.

"27) The appendix is not mentioned in the text and, for that reason, perhaps not needed.
(I did not read/review the appendix since it was never mentioned)."

The appendix has been removed.

"28) Throughout the numerical experiments: when you refer to RMSE, do you mean
analysis RMSE or forecast RMSE?"

We have corrected the formula and clarified that this is in fact the analysis RMSE. (equation 4.3)

"29) Since this paper is about using shrinkage to localize ensemble filters, I recommend
to revise the title to reflect that localization is a key issue here."

While shrinkage does attempt to apply similar ideas to those under the umbrella term "localization", we believe that the methodology is sufficiently different as to merit being described by its own name; we believe that the title is accurate for the methodology, and thus will keep the name.

==> Stochastic Shrinkage ETKFarx3/Prereview/header.tex <==
\newcommand\1{\one}
\def\!#1{\mathcal{#1}}
\def\*#1{\boldsymbol{\mathbf{#1}}}
\def\|#1{\textnormal{#1}}
\def\##1{\mathpzc{#1}}
\renewcommand{\Re}{\mathds{R}}

\def\det#1{\left\lvert#1\right\rvert}
\def\norm#1{\left\lVert#1\right\rVert}
\def\diff#1{\mathrm{d}#1}
\def\sgn{\text{sgn}}

\def\pss#1#2{\prescript{}{#1}{#2}}
\def\psss#1#2#3{\prescript{#1}{#2}{#3}}

\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\tr}{tr}

\newcommand{\C}[2]{\*\Sigma_{#1#2}}
\newcommand{\Ct}[2]{\widetilde{\*\Sigma}_{#1#2}}
\newcommand{\Bt}{\widetilde{\*B}}

\newcommand{\xf}{X^\|f}
\newcommand{\cxf}{\!X^\|f}
\newcommand{\bxf}{\*X^\|f}


%\DeclareMathOperator{\tr}{tr}

\newcommand{\Id}{\mathbf{I}}
\newcommand{\R}{\mathbf{R}}
\renewcommand{\S}{\mathbf{S}}
\newcommand{\transp}{\mathsf{T}}
\newcommand{\Tp}{\mathsf{T}}

\newtheorem{remark}{Remark}

\usepackage{caption}
\usepackage{subcaption}

==> Stochastic Shrinkage ETKFarx3/Prereview2/header.tex <==
\newcommand\1{\one}
\def\!#1{\mathcal{#1}}
\def\*#1{\boldsymbol{\mathbf{#1}}}
\def\|#1{\textnormal{#1}}
\def\##1{\mathpzc{#1}}
\renewcommand{\Re}{\mathds{R}}

\def\det#1{\left\lvert#1\right\rvert}
\def\norm#1{\big\lVert#1\big\rVert}
\def\diff#1{\mathrm{d}#1}
\def\sgn{\text{sgn}}

\def\pss#1#2{\prescript{}{#1}{#2}}
\def\psss#1#2#3{\prescript{#1}{#2}{#3}}

\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\tr}{tr}

\newcommand{\C}[2]{\*\Sigma_{#1#2}}
\newcommand{\Ct}[2]{\widetilde{\*\Sigma}_{#1#2}}
\newcommand{\Bt}{\widetilde{\*B}}

\newcommand{\xf}{X^\|f}
\newcommand{\cxf}{\!X^\|f}
\newcommand{\bxf}{\*X^\|f}


%\DeclareMathOperator{\tr}{tr}

\newcommand{\Id}{\mathbf{I}}
\newcommand{\R}{\mathbf{R}}
\renewcommand{\S}{\mathbf{S}}
\newcommand{\transp}{\mathsf{T}}
\newcommand{\Tp}{\mathsf{T}}

\newtheorem{remark}{Remark}

\usepackage{caption}
\usepackage{subcaption}

==> Stochastic Shrinkage ETKFarx3/Prereview2/responsetorev.tex <==
Response to reviewer 1

"Concepts like KL Kullback-Leibler divergence are not necessarily familiar to atmospheric scientists and this applies to other concepts in the ms. The same applies for the Rao-Blackwellized Ledoit-Wolf (RBLW) estimator."

Answer: The explanation of the RBLW estimator has been substantially expanded in section 2. A line has been added to indicate that the low KL divergence would indicate an ensemble representative of the truth.

"The opinion of this reviewer is that the present manuscript is much more suitable to a scientific computational journal such as SIAM journal of Scientific Computing as it lacks meteorological specificity. ... As an alternative they should consider testing their method on a  meteorological realistic WRF-LETKF system for experiments with real observations which can be considered a major revision required for acceptance for publication in Tellus."

Tellus A has on multiple occasions published new ensemble Kalman filter methods that were tested on Lorenz '96 and the QGE (For example see "Pavel Sakov and Peter R Oke. A deterministic formulation of the ensemble Kalman filter: an alternative to ensemble square root filters. 2008."). It is our opinion that the manuscript and the methodology is well suited for publication to Tellus A.

Response to reviewer 2:

"1) Throughout, the paper is vague and omits important details. The shrinkage approach
relies heavily on the choice of target matrix P, but the authors do not explain how the
target is/should be chosen and what the effects of a poor choice are. I believe that with
a “poor” choice of target, even a “good” gamma cannot yield good results. For that
reason, localizing the target, which in numerical experiments seems to be based on
climatological estimates, should be carefully tuned, but this is not explained."

Sections 2 and 3 have been significantly expanded to clarify both the background, and the proposed approach. A discussion about the choice of target matrix was added to the end of section 2.

"2) In numerical experiments, the authors discuss several variants of the proposed
shrinkage approach, but the paper would be stronger if the authors also compare to
“classical” localization methods — is the shrinkage approach useful compared to a
“vanilla” LETKF, classically tuned (i.e., varying the localization radius and optimizing
forecast error)? Moreover, the numerical tests are done with relatively simple models
(L95 and QG) and a discussion is necessary as to what conclusions one can draw from
these simplified numerical experiments."

The QG experiments already compare our method against an optimally tuned LETKF with Gaspari-Cohn localization. We have added a line to indicate that the GC radius has been optimally tuned.


"3) Section 2.3: I was looking forward to learning about shrinkage techniques, but I found
myself puzzled at the end of this section. I understand the authors have a lot of
experience with shrinkage methods, but the paper would be more impactful and easier
to read (independently of other papers) if the basic ideas of shrinkage methods would
be explained in more detail. Please consider adding more explanations to this important
background section. Specifically, I am unsure how to “choose” a target matrix P and
what the consequences of specific choices could be (see above)."

As is the reply to point 1, the sections on covariance shrinkage and our methodology have been significantly expanded, and rewritten. It is the authors' hope that readers coming from a meteorology background will now gain a better understanding of the proposed methodology.


"1) Consider using a different greek letter in (2.1), I find this letter hard to read and to use
when taking notes (but this is stylistic and can be neglected)."

We did change the capital "Xi" to the small letter "xi", in hope of improving readability. The authors believe that the letter "Xi" is commonly used for the notation involving model error. (equation 2.1)

"2) P. 4 Lines 21-40: Please explain this approximation in more detail and/or give
references."

The authors have found no reference to this in the literature. The discussion of this approximation has been replaced by a simple statement, as to not distract from the rest of the paper.

"3) P. 4 Line 52: What do you mean by “perfect”? Please be more scientifically accurate
and less colloquial."

We have reworded to "inexact". (See line 66)

"3) P. 5 Line 19: The term “shrinkage” is used here (and again, colloquially referred to
as “a type of”), but it is not yet clear/explained what this is. Please remove or explain."

We have removed this line.

"4) P.5 Lines 60-61: There seems to be some confusion between covariances and
correlations. Please correct."

All terms related to covariance matrices have been changed to "covariances". All terms related to localization have keep the terms "correlation" (1 appearance in the abstract) or "decorrelation" (14 appearances in the text), as this is the correct common terminology when refering to such.

"5) Equation 2.14: Please give more background about how this gamma is chosen, in
particular in what sense this choice is “optimal” (what is optimized here?)."

We have added a line to indicate what this is estimating (see line 107) 

"6) Equation 2.16: It is stated that the choice of gamma is “extremely important”. Please
explain in what way the reader should interpret “extremely important” and what the
advantages are of using (2.16) over (2.14) etc."

We have expanded the discussion regarding the significance of gamma, and regarding the advantages and downsides of the RBLW estimator (see lines 121-141)

"7) P. 7 Lines 6-17: You describe two major issues. How do the proposed algorithms
deal with these issues?"

The text (lines 134 to 141) should now hopefully make it clear that we are describing drawbacks to using our proposed methodology without providing a clear answer as to show these issues can be avoided.

"8) P.7 Lines 18-26: In my experience, the “cut-off”, r, has a drastic influence on the
results. How should r be chosen? How is this done in the numerical experiments?
Please consider adding detailed explanations here."

We have added a line to indicate that the localization radius for GC has been optimally tuned. (see lines 311)

"9) P.7 Lines 38-45: What is “our” uncertainty and why is climatological information
“locally known”? I have trouble interpreting these sentences, please clarify."

"Our uncertainty" refers to the Bayesian interpretation of inference. It is inherently dependent on the knowledge of the agent (be it human or machine) performing the inference, thus "our knowledge" and "our uncertainty". This is the terminology used in some statistical literature. The text "locally known" has been removed and largely replaced by "historical". (see line 158 for example)

"10) P.8 Line 17: There is a contradiction. You assume that you know the covariance,
but you want to get to this covariance using localization. Please clarify this circular
reasoning."

We are not sure as to what this is referring to. We see no contradiction. The target covariance, and thereby all forecast ensembles are known prior to the calculation of the shrinkage covariance estimate.

"11) P.8 Lines 25-16: Consider removing the part about Laplace assumptions. It may be
“obvious” to the authors, but this paragraph is not useful for many of Tellus’ readers."

We agree, this has been removed. 

"12) Equation 3.5: How do you pick gammai? Are there general guidelines, a general
tuning framework etc? Please add some clarification here."

We have added the line that in this paper this is the RBLW estimate of gamma. (line 196)

"13) Your use of remarks (p.11 and 16): Consider not using the “Remark” framework,
which is mathematical and it seems out of place of the rest of this paper."

The remark notation has been removed, and the remarks now appear in-text.

"14) L96 assimilation results: I am not sure what is compared here and what “optimal” is
referring to (lines 31 and 34, p. 13). The paper would be stronger if the authors not only
compare variants of the shrinkage techniques, but also compare to “usual localization,”
e.g., and ETKF or similar algorithm."

The usual localization comparisons are already done with the QGE, see figure 3. We have not shied away from showing that the LETKF under certain configurations does in fact beat our method purely in terms of error (see 308-315)

"15) P.14 Line 26: how are the dynamic ensemble sizes modified? Please explain."

We are not sure what this is referring to. If it is referring to the methodology, then the dynamical ensemble size (N) is fixed for all time. We have not considered the case of a changing dynamical ensemble size. If this is refering to the experiments section (section 4), then the ensemble sized are iterated over, and RMSE (and KL) results are obtained for distinct combinations of N and other factors considered.

"16) P. 14, line 30: why/how are gamma values “produced”? Please explain."

The factor gammai, unless otherwise specified to be constant, is computed with the RBLW estimator (see line 196)

"17) The QG model: I believe this is a model on a 2D domain?"

This is stated in the paper. (line 285)

"18) P.15 Line 11: When you apply Gaspari-Cohn to localize (and thereby define the
target matrix P?), how is the spatial length scale of the Gaspari-Cohn function tuned?"

We have added a line to describe that the localization radius is optimally tuned. (line 311)

"19) P.15 Line 13: “Nature” - do you mean the journal, our environment, or a run with the
model that is used to generate observations? Please specify your terminology more
clearly."

We believe that "Nature" is standard terminology in data assimilation literature, and is used to refer to the "true" physical reality, and more specifically to the "true" physical system under consideration.

"20) P.15, Lines 39-43: This statement about ETKF is wrong (and violated by the L96
setup described in this paper). It is in fact the opposite. During a local analysis, nearby
grid points use a very similar set of observations so that the analysis remains (more or
less) smooth."

While the reviewer's statement might be true for some operational models with very sparse observations, for QGE with dense observations, this is not the authors' experience. A naive local update will simply fail as there will be large discontinuities in the solution, leading to non-physical velocities in the QGE. This might be in large part due to the large observation errors in our experiments, and the relative closeness of the observations, but nonetheless our experimental setup is standard for looking at the QGE (see Sakov and Oke 2008). The reason for the inclusion of an "operational approximation" localization function is to attempt to mimic the behavior the reviewer describes in our formulation, and not have a method that simply does not work (as the alternative would in fact lead to an empty plot). Lines 297-306 have been clarified to explain this phenomenon.


"21) P. 15 Line 46: What do you mean by “unfair”? Please focus on strategies that are
reasonable and that are in scientific use. Applying these is not “unfair”."

We have reworded the sentence to reflect the answer above. (lines 297-306)

"22) Equation 4.7: What happens for k>5/4? What is “const”?"

This is a typo, it should have read "sonst." We have changed it to "otherwise" to be consistent with newer English conventions. (equation 4.7)

"23) P. 16, line 7: “handily beats” — how do I see this from the figure and what does this
mean? Please be more specific in your explanations."

The word handily has been removed and the sentence clarified. (lines 308-326)

"24) P.16 Lines 7-20: Is there a reason for why the shrinkage approach should be
expected to do better for nonlinear observations? The rest of this paper does not make
this point and I am not sure this is justified by the theoretical and numerical
developments."

We have changed the wording to reflect a much weaker state of affair, merely that the methodology can work for non-linear observations. (see lines 319-322)


"25) P. 16 Lines 22-32: Again, how is gamma chosen? I understand the choice is
“extremely important”, but it is not clear how the authors propose to choose gamma."

We believe that this is adequately explained in the paper. (see line 196)

"26) Acknowledgements: I am not aware that this paper has already been reviewed by P.
Sakov and another reviewer, I see it for the first time."

This draft is a resubmission, thus it has already been reviewed and substantially changed once.

"27) The appendix is not mentioned in the text and, for that reason, perhaps not needed.
(I did not read/review the appendix since it was never mentioned)."

The appendix has been removed.

"28) Throughout the numerical experiments: when you refer to RMSE, do you mean
analysis RMSE or forecast RMSE?"

We have corrected the formula and clarified that this is in fact the analysis RMSE. (equation 4.3)

"29) Since this paper is about using shrinkage to localize ensemble filters, I recommend
to revise the title to reflect that localization is a key issue here."

While shrinkage does attempt to apply similar ideas to those under the umbrella term "localization", we believe that the methodology is sufficiently different as to merit being described by its own name; we believe that the title is accurate for the methodology, and thus will keep the name.

==> Stochastic Shrinkage ETKFarx3/Reviews_Tellus_v1/responsetorev.tex <==
Response to reviewer 1

"Concepts like KL Kullback-Leibler divergence are not necessarily familiar to atmospheric scientists and this applies to other concepts in the ms. The same applies for the Rao-Blackwellized Ledoit-Wolf (RBLW) estimator."

Answer: The explanation of the RBLW estimator has been substantially expanded in section 2. A line has been added to indicate that the low KL divergence would indicate an ensemble representative of the truth.

"The opinion of this reviewer is that the present manuscript is much more suitable to a scientific computational journal such as SIAM journal of Scientific Computing as it lacks meteorological specificity. ... As an alternative they should consider testing their method on a  meteorological realistic WRF-LETKF system for experiments with real observations which can be considered a major revision required for acceptance for publication in Tellus."

Tellus A has on multiple occasions published new ensemble Kalman filter methods that were tested on Lorenz '96 and the QGE (For example see "Pavel Sakov and Peter R Oke. A deterministic formulation of the ensemble Kalman filter: an alternative to ensemble square root filters. 2008."). It is our opinion that the manuscript and the methodology is well suited for publication to Tellus A.

Response to reviewer 2:

"1) Throughout, the paper is vague and omits important details. The shrinkage approach
relies heavily on the choice of target matrix P, but the authors do not explain how the
target is/should be chosen and what the effects of a poor choice are. I believe that with
a “poor” choice of target, even a “good” gamma cannot yield good results. For that
reason, localizing the target, which in numerical experiments seems to be based on
climatological estimates, should be carefully tuned, but this is not explained."

Sections 2 and 3 have been significantly expanded to clarify both the background, and the proposed approach. A discussion about the choice of target matrix was added to the end of section 2.

"2) In numerical experiments, the authors discuss several variants of the proposed
shrinkage approach, but the paper would be stronger if the authors also compare to
“classical” localization methods — is the shrinkage approach useful compared to a
“vanilla” LETKF, classically tuned (i.e., varying the localization radius and optimizing
forecast error)? Moreover, the numerical tests are done with relatively simple models
(L95 and QG) and a discussion is necessary as to what conclusions one can draw from
these simplified numerical experiments."

The QG experiments already compare our method against an optimally tuned LETKF with Gaspari-Cohn localization. We have added a line to indicate that the GC radius has been optimally tuned.


"3) Section 2.3: I was looking forward to learning about shrinkage techniques, but I found
myself puzzled at the end of this section. I understand the authors have a lot of
experience with shrinkage methods, but the paper would be more impactful and easier
to read (independently of other papers) if the basic ideas of shrinkage methods would
be explained in more detail. Please consider adding more explanations to this important
background section. Specifically, I am unsure how to “choose” a target matrix P and
what the consequences of specific choices could be (see above)."

As is the reply to point 1, the sections on covariance shrinkage and our methodology have been significantly expanded, and rewritten. It is the authors' hope that readers coming from a meteorology background will now gain a better understanding of the proposed methodology.


"1) Consider using a different greek letter in (2.1), I find this letter hard to read and to use
when taking notes (but this is stylistic and can be neglected)."

We did change the capital "Xi" to the small letter "xi", in hope of improving readability. The authors believe that the letter "Xi" is commonly used for the notation involving model error. (equation 2.1)

"2) P. 4 Lines 21-40: Please explain this approximation in more detail and/or give
references."

The authors have found no reference to this in the literature. The discussion of this approximation has been replaced by a simple statement, as to not distract from the rest of the paper.

"3) P. 4 Line 52: What do you mean by “perfect”? Please be more scientifically accurate
and less colloquial."

We have reworded to "inexact". (See line 66)

"3) P. 5 Line 19: The term “shrinkage” is used here (and again, colloquially referred to
as “a type of”), but it is not yet clear/explained what this is. Please remove or explain."

We have removed this line.

"4) P.5 Lines 60-61: There seems to be some confusion between covariances and
correlations. Please correct."

All terms related to covariance matrices have been changed to "covariances". All terms related to localization have keep the terms "correlation" (1 appearance in the abstract) or "decorrelation" (14 appearances in the text), as this is the correct common terminology when refering to such.

"5) Equation 2.14: Please give more background about how this gamma is chosen, in
particular in what sense this choice is “optimal” (what is optimized here?)."

We have added a line to indicate what this is estimating (see line 107) 

"6) Equation 2.16: It is stated that the choice of gamma is “extremely important”. Please
explain in what way the reader should interpret “extremely important” and what the
advantages are of using (2.16) over (2.14) etc."

We have expanded the discussion regarding the significance of gamma, and regarding the advantages and downsides of the RBLW estimator (see lines 121-141)

"7) P. 7 Lines 6-17: You describe two major issues. How do the proposed algorithms
deal with these issues?"

The text (lines 134 to 141) should now hopefully make it clear that we are describing drawbacks to using our proposed methodology without providing a clear answer as to show these issues can be avoided.

"8) P.7 Lines 18-26: In my experience, the “cut-off”, r, has a drastic influence on the
results. How should r be chosen? How is this done in the numerical experiments?
Please consider adding detailed explanations here."

We have added a line to indicate that the localization radius for GC has been optimally tuned. (see lines 311)

"9) P.7 Lines 38-45: What is “our” uncertainty and why is climatological information
“locally known”? I have trouble interpreting these sentences, please clarify."

"Our uncertainty" refers to the Bayesian interpretation of inference. It is inherently dependent on the knowledge of the agent (be it human or machine) performing the inference, thus "our knowledge" and "our uncertainty". This is the terminology used in some statistical literature. The text "locally known" has been removed and largely replaced by "historical". (see line 158 for example)

"10) P.8 Line 17: There is a contradiction. You assume that you know the covariance,
but you want to get to this covariance using localization. Please clarify this circular
reasoning."

We are not sure as to what this is referring to. We see no contradiction. The target covariance, and thereby all forecast ensembles are known prior to the calculation of the shrinkage covariance estimate.

"11) P.8 Lines 25-16: Consider removing the part about Laplace assumptions. It may be
“obvious” to the authors, but this paragraph is not useful for many of Tellus’ readers."

We agree, this has been removed. 

"12) Equation 3.5: How do you pick gammai? Are there general guidelines, a general
tuning framework etc? Please add some clarification here."

We have added the line that in this paper this is the RBLW estimate of gamma. (line 196)

"13) Your use of remarks (p.11 and 16): Consider not using the “Remark” framework,
which is mathematical and it seems out of place of the rest of this paper."

The remark notation has been removed, and the remarks now appear in-text.

"14) L96 assimilation results: I am not sure what is compared here and what “optimal” is
referring to (lines 31 and 34, p. 13). The paper would be stronger if the authors not only
compare variants of the shrinkage techniques, but also compare to “usual localization,”
e.g., and ETKF or similar algorithm."

The usual localization comparisons are already done with the QGE, see figure 3. We have not shied away from showing that the LETKF under certain configurations does in fact beat our method purely in terms of error (see 308-315)

"15) P.14 Line 26: how are the dynamic ensemble sizes modified? Please explain."

We are not sure what this is referring to. If it is referring to the methodology, then the dynamical ensemble size (N) is fixed for all time. We have not considered the case of a changing dynamical ensemble size. If this is refering to the experiments section (section 4), then the ensemble sized are iterated over, and RMSE (and KL) results are obtained for distinct combinations of N and other factors considered.

"16) P. 14, line 30: why/how are gamma values “produced”? Please explain."

The factor gammai, unless otherwise specified to be constant, is computed with the RBLW estimator (see line 196)

"17) The QG model: I believe this is a model on a 2D domain?"

This is stated in the paper. (line 285)

"18) P.15 Line 11: When you apply Gaspari-Cohn to localize (and thereby define the
target matrix P?), how is the spatial length scale of the Gaspari-Cohn function tuned?"

We have added a line to describe that the localization radius is optimally tuned. (line 311)

"19) P.15 Line 13: “Nature” - do you mean the journal, our environment, or a run with the
model that is used to generate observations? Please specify your terminology more
clearly."

We believe that "Nature" is standard terminology in data assimilation literature, and is used to refer to the "true" physical reality, and more specifically to the "true" physical system under consideration.

"20) P.15, Lines 39-43: This statement about ETKF is wrong (and violated by the L96
setup described in this paper). It is in fact the opposite. During a local analysis, nearby
grid points use a very similar set of observations so that the analysis remains (more or
less) smooth."

While the reviewer's statement might be true for some operational models with very sparse observations, for QGE with dense observations, this is not the authors' experience. A naive local update will simply fail as there will be large discontinuities in the solution, leading to non-physical velocities in the QGE. This might be in large part due to the large observation errors in our experiments, and the relative closeness of the observations, but nonetheless our experimental setup is standard for looking at the QGE (see Sakov and Oke 2008). The reason for the inclusion of an "operational approximation" localization function is to attempt to mimic the behavior the reviewer describes in our formulation, and not have a method that simply does not work (as the alternative would in fact lead to an empty plot). Lines 297-306 have been clarified to explain this phenomenon.


"21) P. 15 Line 46: What do you mean by “unfair”? Please focus on strategies that are
reasonable and that are in scientific use. Applying these is not “unfair”."

We have reworded the sentence to reflect the answer above. (lines 297-306)

"22) Equation 4.7: What happens for k>5/4? What is “const”?"

This is a typo, it should have read "sonst." We have changed it to "otherwise" to be consistent with newer English conventions. (equation 4.7)

"23) P. 16, line 7: “handily beats” — how do I see this from the figure and what does this
mean? Please be more specific in your explanations."

The word handily has been removed and the sentence clarified. (lines 308-326)

"24) P.16 Lines 7-20: Is there a reason for why the shrinkage approach should be
expected to do better for nonlinear observations? The rest of this paper does not make
this point and I am not sure this is justified by the theoretical and numerical
developments."

We have changed the wording to reflect a much weaker state of affair, merely that the methodology can work for non-linear observations. (see lines 319-322)


"25) P. 16 Lines 22-32: Again, how is gamma chosen? I understand the choice is
“extremely important”, but it is not clear how the authors propose to choose gamma."

We believe that this is adequately explained in the paper. (see line 196)

"26) Acknowledgements: I am not aware that this paper has already been reviewed by P.
Sakov and another reviewer, I see it for the first time."

This draft is a resubmission, thus it has already been reviewed and substantially changed once.

"27) The appendix is not mentioned in the text and, for that reason, perhaps not needed.
(I did not read/review the appendix since it was never mentioned)."

The appendix has been removed.

"28) Throughout the numerical experiments: when you refer to RMSE, do you mean
analysis RMSE or forecast RMSE?"

We have corrected the formula and clarified that this is in fact the analysis RMSE. (equation 4.3)

"29) Since this paper is about using shrinkage to localize ensemble filters, I recommend
to revise the title to reflect that localization is a key issue here."

While shrinkage does attempt to apply similar ideas to those under the umbrella term "localization", we believe that the methodology is sufficiently different as to merit being described by its own name; we believe that the title is accurate for the methodology, and thus will keep the name.

==> Stochastic Shrinkage ETKFarx3/header.tex <==
\newcommand\1{\one}
\def\!#1{\mathcal{#1}}
\def\*#1{\boldsymbol{\mathbf{#1}}}
\def\|#1{\textnormal{#1}}
\def\##1{\mathpzc{#1}}
\renewcommand{\Re}{\mathds{R}}

\def\det#1{\left\lvert#1\right\rvert}
\def\norm#1{\big\lVert#1\big\rVert}
\def\diff#1{\mathrm{d}#1}
\def\sgn{\text{sgn}}

\def\pss#1#2{\prescript{}{#1}{#2}}
\def\psss#1#2#3{\prescript{#1}{#2}{#3}}

\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\tr}{tr}

\newcommand{\C}[2]{\*\Sigma_{#1#2}}
\newcommand{\Ct}[2]{\widetilde{\*\Sigma}_{#1#2}}
\newcommand{\Bt}{\widetilde{\*B}}

\newcommand{\xf}{X^\|f}
\newcommand{\cxf}{\!X^\|f}
\newcommand{\bxf}{\*X^\|f}


%\DeclareMathOperator{\tr}{tr}

\newcommand{\Id}{\mathbf{I}}
\newcommand{\R}{\mathbf{R}}
\renewcommand{\S}{\mathbf{S}}
\newcommand{\transp}{\mathsf{T}}
\newcommand{\Tp}{\mathsf{T}}

\newtheorem{remark}{Remark}

\usepackage{caption}
\usepackage{subcaption}
